Heuristic Voting as Ordinal Dominance Strategies

Decision making under uncertainty is a key component of many AI settings, and in particular of voting scenarios where strategic agents are trying to reach a joint decision. The common approach to handle uncertainty is by maximizing expected utility, which requires a cardinal utility function as well as detailed probabilistic information. However, often such probabilities are not easy to estimate or apply. To this end, we present a framework that allows "shades of gray" of likelihood without probabilities. Specifically, we create a hierarchy of sets of world states based on a prospective poll, with inner sets contain more likely outcomes. This hierarchy of likelihoods allows us to define what we term ordinally-dominated strategies. We use this approach to justify various known voting heuristics as bounded-rational strategies.

==> sensor_fig.tex <==
%\documentclass[]{article}
%\usepackage{tikz}
%%\usepackage{tikz}%,fullpage}
%\usetikzlibrary{arrows,%
                %petri,%
                %topaths,calc,decorations.pathreplacing}
%\usepackage{tkz-berge}
%\usepackage[position=top]{subfig}
%\tikzset{
  %font={\fontsize{14pt}{12}\selectfont}}
%
%\begin{document}
%\begin{figure}
\centering
\subfloat[Entry routes]{ %\label{fig:routes}
\begin{tikzpicture}[scale=0.7,transform shape]


\tikzstyle{sensor}=[draw=black,fill=white,
inner sep=0pt,minimum size=5mm]

\draw[thick] (0,0) -- (2,0);
\draw[thick] (3,0) -- (5,0);
\draw[thick] (6.5,0) -- (9,0);
	\node at (2.5,-0.5) {$x_4$};
	\node at (5.75,-0.5) [sensor] {$x_2$};
	\node at (2.6,1.9) [sensor] {$x_1$};
	\node at (7,1.6) [sensor] {$x_3$};
 %\tikzstyle{VertexStyle}=[]
\node at (8.5,1.1) {$p'$};
\draw[->] (9,1.5) .. controls (6.5,1.4)   .. (6.1,-1);
\node at (4,1.7) {$p$};
\draw[->] (0,2.3) .. controls (5,2.3)   .. (5.3,-1);
\node at (0.5,1.6) {$p'''$};
\node at (0.5,0.6) {$p''$};

\draw[dashed,->] (0,2) .. controls (2.4,2)   .. (3,-1);	
\draw[dashed,->] (0,1) .. controls (2,1)  .. (2.25,-1);
	
\end{tikzpicture}
}
\subfloat[Information structure]{% \label{fig:S}
\begin{tikzpicture}[scale=0.45,transform shape]
\fill[white] (-1,0) rectangle (4,0);
\fill[black!15!white] (0,0) rectangle (2,3);
\fill[black!30!white] (0.05,1) rectangle (1.9,2.9);
\fill[black!40!white] (0.1,2) rectangle (1.8,2.8);
\draw[thin] (0,0) rectangle (2,3);
\draw[thin] (0.05,1) rectangle (1.9,2.9);
\draw[thin] (0.1,2) rectangle (1.8,2.8);

\node at (1,2.5) {$p^0$};
\node at (1,1.5) {$p,p'$};
\node at (1,0.5) {$p'',p'''$};

%\node at (-0.7,2.5) {$S_1$};
\draw [decorate,decoration={brace,amplitude=4pt},xshift=0pt,yshift=0pt] (2.1,3) -- (2.1,1) node [black,midway,xshift=0.6cm] { $S_2$};
\draw [decorate,decoration={brace,amplitude=4pt},xshift=0pt,yshift=0pt] (-0.1,0) -- (-0.1,3) node [black,midway,xshift=-0.6cm] { $S_3$};



\node at (3.5,2.5) {$H_1$};
\Vertex[x=4.5,y=2.5,L=$c^+$]{a}
\Vertex[x=6,y=2.5,L=$c^-$]{b}
\Vertex[x=7.5,y=2.5,L=$c^0$]{c}


\node at (3.5,1.5) {$H_2$};
\Vertex[x=4.5,y=1.5,L=$c^+$]{a}
\Vertex[x=6,y=1.5,L=$c^-$]{b}
\Vertex[x=7.5,y=1.5,L=$c^0$]{c}
\Edge(a)(b)



\node at (3.5,0.5) {$H_3$};
\Vertex[x=4.5,y=0.5,L=$c^+$]{a}
\Vertex[x=6,y=0.5,L=$c^-$]{b}
\Vertex[x=7.5,y=0.5,L=$c^0$]{c}
\Edge(a)(b)


\end{tikzpicture}
}
%
%\end{figure}
%
%\end{document}

